ENHANCE (ENriching Health data by ANnotations of Crowd and Experts): A case study for skin lesion classification

We present ENHANCE, an open dataset with multiple annotations to complement the existing ISIC and PH2 skin lesion classification datasets. This dataset contains annotations of visual ABC (asymmetry, border, colour) features from non-expert annotation sources: undergraduate students, crowd workers from Amazon MTurk and classic image processing algorithms. In this paper we first analyse the correlations between the annotations and the diagnostic label of the lesion, as well as study the agreement between different annotation sources. Overall we find weak correlations of non-expert annotations with the diagnostic label, and low agreement between different annotation sources. We then study multi-task learning (MTL) with the annotations as additional labels, and show that non-expert annotations can improve (ensembles of) state-of-the-art convolutional neural networks via MTL. We hope that our dataset can be used in further research into multiple annotations and/or MTL. All data and models are available on Github: https://github.com/raumannsr/ENHANCE.

==> appendices/app_lr.tex <==
\added{We determined a value of 2e-5 as a reasonable learning rate by evaluating six learning rates on the baseline VGG16 model (see table below).}
\begin{table}[ht]
    \centering
    \input{tables/learning_rates_table}
    \caption{AUCx100 performances of six learning rates on the baseline VGG16 model.}
    \label{tab:lr_table}
\end{table}

==> archive/reviews.tex <==
Questions
2. Please provide a summary of the paper (a few lines)
In this paper, the authors validated that multi-task learning with crowd sourced labels (border, color and asymmetry, i.e. features related to skin lesions) helps boost the performance of skin lesion classification, compared to their baseline model based on binary classification with diagnostic labels.
3. Please list the major strengths of the paper; you should write about a novel formulation, an original way to use data, demonstration of clinical feasibility, a novel application, or anything else that is a strong aspect of this work (bulleted list)
The paper discussed from a practical angel about utilizing crowdsourced labels for skin lesion classification. Collecting labels for border, color and asymmetry is cost effective and can easily scale up. Therefore, I think the paper has good potential and practical merits.
4. Please list the major weaknesses of the paper (bulleted list).
1. To verify the effectiveness of multi-task learning with crowdsourced labels, I think the authors need to experiment on the number of additional training images with diagnostic labels that can achieve similar performance boost on test set. The proposed method would have an advantage if a large amount of additional diagnostic labels are required to achieve the same performance. However, I don't see sufficient experimental results in the paper that can convince me on that.
2. I am also concerned with the lack of comparison to state-of-the-art methods, besides the simple baseline model in the paper.
5. Please rate the clarity and organization of this paper
Satisfactory
6. Please provide detailed and constructive comments for the authors. Please also refer to our Reviewer's guide on what makes a good review: https://miccai2020.org/en/REVIEWER-GUIDELINES.html
The layout of the paper is more like a technical report. I think many of the listed TO DO tasks (for example, tune a dedicated network for skin lesion classification, instead of freezing weights pre-trained on ImageNet) in Discussion and Conclusion section needs to be finished to draw confident conclusions.
Reviewer #3
Questions
2. Please provide a summary of the paper (a few lines)
The paper proposes a multi-task learning with crowdsourced features for skin lesion diagnosis.
3. Please list the major strengths of the paper; you should write about a novel formulation, an original way to use data, demonstration of clinical feasibility, a novel application, or anything else that is a strong aspect of this work (bulleted list)
The method is interesting.
4. Please list the major weaknesses of the paper (bulleted list).
1. The paper is of poor organization.
2. More experiments should be included to validate the effectiveness of the proposed approach. (comparison with the sota may be helpful)
5. Please rate the clarity and organization of this paper
Satisfactory
6. Please provide detailed and constructive comments for the authors. Please also refer to our Reviewer's guide on what makes a good review: https://miccai2020.org/en/REVIEWER-GUIDELINES.html
1. The approach is interesting, but the experimental section is unsatisfactory. More experiments should be included, such as ablation study (combination of the features) and comparison with sota on ISIC 2017.
2. The paper is of poor organization. The Fig. 2 is too large.
Reviewer #5
Questions
2. Please provide a summary of the paper (a few lines)
This paper aim at classifying skin lesions as malignant or not using binary classifier. It study the possibility of providing an alternative for label annotations by getting aid from "crowdsourcing" information. That is collecting additional primitive visual features (i.e color or shape) form non-experts (students). Crowdsourcing features are used in the learning process and formalized as multi-task framework. Results show slight improvement with +3.1% AUC improvement w.r.t a baseline model.
3. Please list the major strengths of the paper; you should write about a novel formulation, an original way to use data, demonstration of clinical feasibility, a novel application, or anything else that is a strong aspect of this work (bulleted list)
Asking crowd about visual features, such as asymmetrical shape of the lesion, border irregularity, color of the assessed lesion, of the image and integrating them in the learning process.

4. Please list the major weaknesses of the paper (bulleted list).
1. This study do not clearly show the main contribution of crowdsourcing features at the level of improving the prediction.
2. The experimental part and analysis is weak. It lack the comparison with state of the art. It does not emphasis on the importance of the crowd primitive features that are additionally used.
3. The benefit of formalizing the problem into multi-task (binary classification and annotation-regression task) is not clear. For instance, why the crowd features are not fused instead? Why, instead of doing binary classification plus predicting one of the crowd features (either asymmetry, border or color), not altogether (crowd features) are predicted plus binary classification?
4. Why the performance of the main baseline is not enhanced and well fine-tuned? Why the contribution of Crowdsourcing features is not studied on the top of recent state of the art methods?
5. The improvement of 3.1% over the test data, which contains only 250 samples, is not that significant.
5. Please rate the clarity and organization of this paper
Satisfactory
6. Please provide detailed and constructive comments for the authors. Please also refer to our Reviewer's guide on what makes a good review: https://miccai2020.org/en/REVIEWER-GUIDELINES.html
1. The paper is satisfactory written and easy to follow. It follow typical structure organization. The goal of the authors is clear.

2. I disagree with some part of the introduction: such as "ML is not widely used in healthcare", this not true, machine learning is heavily studied in healthcare and most recent methods address the challenge of lack of annotated data by switching to weakly and semi-supervised methods.

3. Reference [13] is arXiv and in Reference [17] the list of authors is too big, it can be limited to three and the rest can be written as et. al.

4. Related work section is missing or not integrated with the introduction part. The authors are encouraged to clearly run a related work study and emphasis on their choices.

5. The mathematical formalization of the main objective function is needed.

6. Experimental validation should be further studied and expanded. It is more preferable to build a baseline on the top of the most recent methods and then to integrate the crowdsourcing features and study their contribution.


Please provide your assessment of this work, taking into account all reviews.
Experiments are "weak" and "not convincing" enough (R1, R3, and R5) and related work and comparison with SOTA are missing (R1, R3). While the paper targets an interesting topic to the Medical Image Computing, I rather agree with the concerns of the reviewers and I think the paper is not ready for publication in its current form.

==> sec_acknowledgements.tex <==
We would like to acknowledge all students and crowd workers who have contributed to this project with image annotation. We gratefully acknowledge financial support from the Netherlands Organization for Scientific Research (NWO), grant no. 023.014.010.

==> sec_research_questions.tex <==
We study the quality of non-expert annotations from different viewpoints: the discriminability of ABC features for diagnosis, the inter agreement level for A, B and C feature between the different annotation sources, and the performance benefits from using multiple annotations in MTL. This investigation addresses the following specific questions:
\begin{enumerate}
  \item How discriminative are ABC features for diagnosis?
  \item What is the inter agreement level for A, B and C feature between the different annotation sources?
  \item How can CNN performance benefit from using multiple annotations?
\end{enumerate}

==> sec_technical_aspects.tex <==
When using automated annotation, the ground truth masks'  boundaries are essential for accurately annotating asymmetry, border irregularity, and color characteristics. However, we see a wide variation in the given mask boundary definitions: ranging from precisely defined to more loose boundary ones. Besides, some masks have clipped boundaries. (Fig.~\ref{BINARY_MASKS}). In the asymmetry annotation algorithm, we do not use the latter (30 ISIC and 35 PH2 based cases). Also, the border annotation algorithm cannot determine the distance between border and edge with some clipped masks (4 ISIC based cases).

\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/precise_loose_clipped_masks.eps}
    \caption{Examples of masks with precise (left), loose (middle), and clipped boundary (right) descriptions}
    \label{BINARY_MASKS}
\end{figure}

==> tables/inception_table_auc.tex <==
\begin{tabular}{lrrr}
\toprule
      Type &  Asymmetry &  Border &  Color \\
\midrule
   Student &     0.8403 &  0.8521 & 0.8570 \\
     Crowd &     0.8548 &  0.8608 & 0.8512 \\
 Automated &     0.8540 &  0.8477 & 0.8503 \\
\bottomrule
\end{tabular}


==> tables/learning_rates_table.tex <==
\begin{tabular}{lll}
\hline
     Seed & Learning rate & AUCx100 \\
\hline
    1970 &  $2.0\mathrm{e}{-5}$  &  79.9  \\
    1970 &  $1.0\mathrm{e}{-5}$  &  75.6  \\
    1970 &  $2.0\mathrm{e}{-4}$  &  50.0  \\
    1970 &  $1.0\mathrm{e}{-4}$  &  50.0  \\
    1970 &  $2.0\mathrm{e}{-3}$  &  50.0  \\
    1970 &  $1.0\mathrm{e}{-3}$  &  50.0  \\
    1972 &  $2.0\mathrm{e}{-5}$  &  76.6  \\
    1972 &  $1.0\mathrm{e}{-5}$  &  78.9  \\
    1972 &  $2.0\mathrm{e}{-4}$  &  50.0  \\
    1972 &  $1.0\mathrm{e}{-4}$  &  50.0  \\
    1972 &  $2.0\mathrm{e}{-3}$  &  50.0  \\
    1972 &  $1.0\mathrm{e}{-3}$  &  50.0  \\
\hline
\end{tabular}

==> tables/pearson_table.tex <==
\begin{tabular}{llll}
\toprule
    Configuration & Asymmetry &  Border &  Color \\
\midrule
    Student-Crowd &    0.3527 & -0.0474 & 0.2918 \\
 Student-Computer &    0.0554 &  0.0282 & 0.2335 \\
   Crowd-Computer &    0.0963 & -0.0459 & 0.2566 \\
  Expert-Computer &    0.0949 &    n.a. & 0.0681 \\
     Expert-Crowd &      todo &    n.a. &   todo \\
\bottomrule
\end{tabular}


==> tables/resnet_table_auc.tex <==
\begin{tabular}{lrrr}
\toprule
      Type &  Asymmetry &  Border &  Color \\
\midrule
   Student &     0.8576 &  0.8462 & 0.8444 \\
     Crowd &     0.8479 &  0.8528 & 0.8420 \\
 Automated &     0.8573 &  0.8526 & 0.8451 \\
\bottomrule
\end{tabular}


==> tables/vgg16_table_auc.tex <==
\begin{tabular}{lrrr}
\toprule
      Type &  Asymmetry &  Border &  Color \\
\midrule
   Student &     0.8030 &  0.7989 & 0.7885 \\
     Crowd &     0.8087 &  0.7860 & 0.7857 \\
 Automated &     0.7900 &  0.7882 & 0.7905 \\
\bottomrule
\end{tabular}

